Multi-Variable Conformal Prediction: Optimizing Prediction Sets using Multiple Calibration Variables

Split conformal prediction constructs prediction sets with finite-sample coverage guarantees, but its calibration stage is limited to adjusting a single threshold parameter. Hence, the shape of the prediction sets must be fixed beforehand, typically by fitting it on a reserved part of the calibration data. We introduce multi-variable conformal prediction (MCP), a framework that jointly optimizes and calibrates multiple prediction-set parameters in a single optimization problem, eliminating calibration data split without sacrificing finite-sample coverage guarantees. Building on scenario theory, a principled framework for certifying data-driven decisions, we propose two tractable variants: RemMCP, grounded in constrained optimization with constraint removal, which generalizes split conformal prediction; and RelMCP, based on penalized optimization with constraint relaxation, which also supports non-convex problems, albeit at a higher computational cost. In experiments with ellipsoidal and multi-modal prediction sets, RemMCP and a heuristic, adaptive version of RelMCP consistently meet the target coverage, with lower variance across calibration runs than baselines with calibration data split, and in most settings with smaller or comparable prediction sets.

==> figures/fig_helpers/beta_coords_ncal1000_eps5_nq1_rho20.tex <==
0.90000 0.00000
0.90025 0.00000
0.90050 0.00000
0.90075 0.00000
0.90100 0.00000
0.90125 0.00000
0.90150 0.00000
0.90175 0.00000
0.90201 0.00000
0.90226 0.00000
0.90251 0.00000
0.90276 0.00000
0.90301 0.00000
0.90326 0.00000
0.90351 0.00000
0.90376 0.00000
0.90401 0.00000
0.90426 0.00000
0.90451 0.00000
0.90476 0.00000
0.90501 0.00000
0.90526 0.00000
0.90551 0.00000
0.90576 0.00000
0.90602 0.00000
0.90627 0.00000
0.90652 0.00000
0.90677 0.00000
0.90702 0.00000
0.90727 0.00000
0.90752 0.00000
0.90777 0.00000
0.90802 0.00000
0.90827 0.00000
0.90852 0.00000
0.90877 0.00000
0.90902 0.00000
0.90927 0.00000
0.90952 0.00000
0.90977 0.00000
0.91003 0.00000
0.91028 0.00000
0.91053 0.00000
0.91078 0.00000
0.91103 0.00000
0.91128 0.00000
0.91153 0.00000
0.91178 0.00000
0.91203 0.00000
0.91228 0.00000
0.91253 0.00000
0.91278 0.00000
0.91303 0.00000
0.91328 0.00000
0.91353 0.00000
0.91378 0.00000
0.91404 0.00000
0.91429 0.00000
0.91454 0.00000
0.91479 0.00000
0.91504 0.00000
0.91529 0.00000
0.91554 0.00000
0.91579 0.00000
0.91604 0.00000
0.91629 0.00000
0.91654 0.00000
0.91679 0.00000
0.91704 0.00000
0.91729 0.00000
0.91754 0.00000
0.91779 0.00000
0.91805 0.00000
0.91830 0.00000
0.91855 0.00000
0.91880 0.00000
0.91905 0.00000
0.91930 0.00000
0.91955 0.00000
0.91980 0.00000
0.92005 0.00000
0.92030 0.00000
0.92055 0.00000
0.92080 0.00000
0.92105 0.00000
0.92130 0.00000
0.92155 0.00000
0.92180 0.00000
0.92206 0.00000
0.92231 0.00000
0.92256 0.00000
0.92281 0.00000
0.92306 0.00000
0.92331 0.00000
0.92356 0.00000
0.92381 0.00000
0.92406 0.00000
0.92431 0.00000
0.92456 0.00000
0.92481 0.00000
0.92506 0.00000
0.92531 0.00000
0.92556 0.00000
0.92581 0.00000
0.92607 0.00000
0.92632 0.00000
0.92657 0.00000
0.92682 0.00000
0.92707 0.00000
0.92732 0.00000
0.92757 0.00000
0.92782 0.00000
0.92807 0.00000
0.92832 0.00000
0.92857 0.00000
0.92882 0.00000
0.92907 0.00000
0.92932 0.00000
0.92957 0.00000
0.92982 0.00000
0.93008 0.00000
0.93033 0.00000
0.93058 0.00000
0.93083 0.00000
0.93108 0.00000
0.93133 0.00000
0.93158 0.00000
0.93183 0.00000
0.93208 0.00000
0.93233 0.00000
0.93258 0.00000
0.93283 0.00000
0.93308 0.00000
0.93333 0.00000
0.93358 0.00000
0.93383 0.00000
0.93409 0.00000
0.93434 0.00000
0.93459 0.00000
0.93484 0.00000
0.93509 0.00000
0.93534 0.00000
0.93559 0.00000
0.93584 0.00000
0.93609 0.00000
0.93634 0.00000
0.93659 0.00000
0.93684 0.00000
0.93709 0.00000
0.93734 0.00000
0.93759 0.00000
0.93784 0.00000
0.93810 0.00000
0.93835 0.00000
0.93860 0.00000
0.93885 0.00000
0.93910 0.00000
0.93935 0.00000
0.93960 0.00000
0.93985 0.00000
0.94010 0.00000
0.94035 0.00000
0.94060 0.00000
0.94085 0.00000
0.94110 0.00000
0.94135 0.00000
0.94160 0.00000
0.94185 0.00000
0.94211 0.00000
0.94236 0.00000
0.94261 0.00000
0.94286 0.00000
0.94311 0.00001
0.94336 0.00001
0.94361 0.00001
0.94386 0.00001
0.94411 0.00001
0.94436 0.00001
0.94461 0.00001
0.94486 0.00002
0.94511 0.00002
0.94536 0.00002
0.94561 0.00003
0.94586 0.00003
0.94612 0.00004
0.94637 0.00005
0.94662 0.00006
0.94687 0.00007
0.94712 0.00008
0.94737 0.00009
0.94762 0.00011
0.94787 0.00013
0.94812 0.00015
0.94837 0.00017
0.94862 0.00020
0.94887 0.00024
0.94912 0.00028
0.94937 0.00033
0.94962 0.00039
0.94987 0.00046
0.95013 0.00053
0.95038 0.00062
0.95063 0.00073
0.95088 0.00085
0.95113 0.00100
0.95138 0.00117
0.95163 0.00136
0.95188 0.00159
0.95213 0.00185
0.95238 0.00215
0.95263 0.00251
0.95288 0.00292
0.95313 0.00339
0.95338 0.00394
0.95363 0.00458
0.95388 0.00531
0.95414 0.00616
0.95439 0.00714
0.95464 0.00827
0.95489 0.00957
0.95514 0.01107
0.95539 0.01280
0.95564 0.01478
0.95589 0.01706
0.95614 0.01968
0.95639 0.02268
0.95664 0.02612
0.95689 0.03006
0.95714 0.03457
0.95739 0.03973
0.95764 0.04562
0.95789 0.05235
0.95815 0.06001
0.95840 0.06875
0.95865 0.07870
0.95890 0.09002
0.95915 0.10287
0.95940 0.11747
0.95965 0.13403
0.95990 0.15280
0.96015 0.17404
0.96040 0.19807
0.96065 0.22523
0.96090 0.25587
0.96115 0.29044
0.96140 0.32937
0.96165 0.37318
0.96190 0.42243
0.96216 0.47774
0.96241 0.53978
0.96266 0.60929
0.96291 0.68709
0.96316 0.77406
0.96341 0.87118
0.96366 0.97949
0.96391 1.10016
0.96416 1.23442
0.96441 1.38361
0.96466 1.54920
0.96491 1.73275
0.96516 1.93594
0.96541 2.16058
0.96566 2.40859
0.96591 2.68203
0.96617 2.98309
0.96642 3.31409
0.96667 3.67748
0.96692 4.07583
0.96717 4.51186
0.96742 4.98838
0.96767 5.50834
0.96792 6.07480
0.96817 6.69090
0.96842 7.35987
0.96867 8.08500
0.96892 8.86963
0.96917 9.71712
0.96942 10.63083
0.96967 11.61408
0.96992 12.67012
0.97018 13.80210
0.97043 15.01300
0.97068 16.30564
0.97093 17.68257
0.97118 19.14604
0.97143 20.69795
0.97168 22.33979
0.97193 24.07257
0.97218 25.89673
0.97243 27.81212
0.97268 29.81792
0.97293 31.91252
0.97318 34.09353
0.97343 36.35766
0.97368 38.70069
0.97393 41.11738
0.97419 43.60144
0.97444 46.14550
0.97469 48.74105
0.97494 51.37842
0.97519 54.04679
0.97544 56.73417
0.97569 59.42744
0.97594 62.11236
0.97619 64.77367
0.97644 67.39512
0.97669 69.95960
0.97694 72.44925
0.97719 74.84558
0.97744 77.12968
0.97769 79.28236
0.97794 81.28436
0.97820 83.11661
0.97845 84.76042
0.97870 86.19776
0.97895 87.41153
0.97920 88.38580
0.97945 89.10612
0.97970 89.55974
0.97995 89.73592
0.98020 89.62615
0.98045 89.22437
0.98070 88.52719
0.98095 87.53404
0.98120 86.24733
0.98145 84.67248
0.98170 82.81802
0.98195 80.69555
0.98221 78.31970
0.98246 75.70795
0.98271 72.88053
0.98296 69.86011
0.98321 66.67159
0.98346 63.34167
0.98371 59.89856
0.98396 56.37150
0.98421 52.79033
0.98446 49.18503
0.98471 45.58521
0.98496 42.01970
0.98521 38.51600
0.98546 35.09994
0.98571 31.79521
0.98596 28.62304
0.98622 25.60189
0.98647 22.74726
0.98672 20.07149
0.98697 17.58368
0.98722 15.28973
0.98747 13.19235
0.98772 11.29126
0.98797 9.58334
0.98822 8.06293
0.98847 6.72216
0.98872 5.55126
0.98897 4.53896
0.98922 3.67288
0.98947 2.93989
0.98972 2.32650
0.98997 1.81919
0.99023 1.40474
0.99048 1.07047
0.99073 0.80446
0.99098 0.59575
0.99123 0.43440
0.99148 0.31160
0.99173 0.21967
0.99198 0.15203
0.99223 0.10317
0.99248 0.06857
0.99273 0.04457
0.99298 0.02828
0.99323 0.01750
0.99348 0.01053
0.99373 0.00615
0.99398 0.00348
0.99424 0.00190
0.99449 0.00100
0.99474 0.00051
0.99499 0.00024
0.99524 0.00011
0.99549 0.00005
0.99574 0.00002
0.99599 0.00001
0.99624 0.00000
0.99649 0.00000
0.99674 0.00000
0.99699 0.00000
0.99724 0.00000
0.99749 0.00000
0.99774 0.00000
0.99799 0.00000
0.99825 0.00000
0.99850 0.00000
0.99875 0.00000
0.99900 0.00000
0.99925 0.00000
0.99950 0.00000
0.99975 0.00000
1.00000 0.00000


==> figures/fig_helpers/beta_coords_ncal1000_eps5_nq1_rho49.tex <==
0.65000 0.00000
0.65176 0.00000
0.65352 0.00000
0.65528 0.00000
0.65704 0.00000
0.65879 0.00000
0.66055 0.00000
0.66231 0.00000
0.66407 0.00000
0.66583 0.00000
0.66759 0.00000
0.66935 0.00000
0.67111 0.00000
0.67286 0.00000
0.67462 0.00000
0.67638 0.00000
0.67814 0.00000
0.67990 0.00000
0.68166 0.00000
0.68342 0.00000
0.68518 0.00000
0.68693 0.00000
0.68869 0.00000
0.69045 0.00000
0.69221 0.00000
0.69397 0.00000
0.69573 0.00000
0.69749 0.00000
0.69925 0.00000
0.70101 0.00000
0.70276 0.00000
0.70452 0.00000
0.70628 0.00000
0.70804 0.00000
0.70980 0.00000
0.71156 0.00000
0.71332 0.00000
0.71508 0.00000
0.71683 0.00000
0.71859 0.00000
0.72035 0.00000
0.72211 0.00000
0.72387 0.00000
0.72563 0.00000
0.72739 0.00000
0.72915 0.00000
0.73090 0.00000
0.73266 0.00000
0.73442 0.00000
0.73618 0.00000
0.73794 0.00000
0.73970 0.00000
0.74146 0.00000
0.74322 0.00000
0.74497 0.00000
0.74673 0.00000
0.74849 0.00000
0.75025 0.00000
0.75201 0.00000
0.75377 0.00000
0.75553 0.00000
0.75729 0.00000
0.75905 0.00000
0.76080 0.00000
0.76256 0.00000
0.76432 0.00000
0.76608 0.00000
0.76784 0.00000
0.76960 0.00000
0.77136 0.00000
0.77312 0.00000
0.77487 0.00000
0.77663 0.00000
0.77839 0.00000
0.78015 0.00000
0.78191 0.00000
0.78367 0.00000
0.78543 0.00000
0.78719 0.00000
0.78894 0.00000
0.79070 0.00000
0.79246 0.00000
0.79422 0.00000
0.79598 0.00000
0.79774 0.00000
0.79950 0.00000
0.80126 0.00000
0.80302 0.00000
0.80477 0.00000
0.80653 0.00000
0.80829 0.00000
0.81005 0.00000
0.81181 0.00000
0.81357 0.00000
0.81533 0.00000
0.81709 0.00000
0.81884 0.00000
0.82060 0.00000
0.82236 0.00000
0.82412 0.00000
0.82588 0.00000
0.82764 0.00000
0.82940 0.00000
0.83116 0.00000
0.83291 0.00000
0.83467 0.00000
0.83643 0.00000
0.83819 0.00000
0.83995 0.00000
0.84171 0.00000
0.84347 0.00000
0.84523 0.00000
0.84698 0.00000
0.84874 0.00000
0.85050 0.00000
0.85226 0.00000
0.85402 0.00000
0.85578 0.00000
0.85754 0.00000
0.85930 0.00000
0.86106 0.00000
0.86281 0.00000
0.86457 0.00000
0.86633 0.00000
0.86809 0.00000
0.86985 0.00000
0.87161 0.00000
0.87337 0.00000
0.87513 0.00000
0.87688 0.00000
0.87864 0.00000
0.88040 0.00000
0.88216 0.00000
0.88392 0.00000
0.88568 0.00000
0.88744 0.00000
0.88920 0.00000
0.89095 0.00000
0.89271 0.00000
0.89447 0.00000
0.89623 0.00000
0.89799 0.00000
0.89975 0.00000
0.90151 0.00000
0.90327 0.00001
0.90503 0.00003
0.90678 0.00006
0.90854 0.00016
0.91030 0.00039
0.91206 0.00092
0.91382 0.00212
0.91558 0.00481
0.91734 0.01061
0.91910 0.02281
0.92085 0.04777
0.92261 0.09732
0.92437 0.19264
0.92613 0.37006
0.92789 0.68905
0.92965 1.24187
0.93141 2.16331
0.93317 3.63662
0.93492 5.88936
0.93668 9.17125
0.93844 13.70589
0.94020 19.61364
0.94196 26.81320
0.94372 34.92614
0.94548 43.22427
0.94724 50.66656
0.94899 56.05763
0.95075 58.31928
0.95251 56.80897
0.95427 51.57078
0.95603 43.39960
0.95779 33.65856
0.95955 23.89663
0.96131 15.41438
0.96307 8.95614
0.96482 4.64120
0.96658 2.12080
0.96834 0.84329
0.97010 0.28728
0.97186 0.08232
0.97362 0.01941
0.97538 0.00367
0.97714 0.00054
0.97889 0.00006
0.98065 0.00000
0.98241 0.00000
0.98417 0.00000
0.98593 0.00000
0.98769 0.00000
0.98945 0.00000
0.99121 0.00000
0.99296 0.00000
0.99472 0.00000
0.99648 0.00000
0.99824 0.00000
1.00000 0.00000


==> figures/fig_helpers/beta_coords_ncal2000_eps5_nq1_rho56.tex <==
0.90000 0.00000
0.90025 0.00000
0.90050 0.00000
0.90075 0.00000
0.90100 0.00000
0.90125 0.00000
0.90150 0.00000
0.90175 0.00000
0.90201 0.00000
0.90226 0.00000
0.90251 0.00000
0.90276 0.00000
0.90301 0.00000
0.90326 0.00000
0.90351 0.00000
0.90376 0.00000
0.90401 0.00000
0.90426 0.00000
0.90451 0.00000
0.90476 0.00000
0.90501 0.00000
0.90526 0.00000
0.90551 0.00000
0.90576 0.00000
0.90602 0.00000
0.90627 0.00000
0.90652 0.00000
0.90677 0.00000
0.90702 0.00000
0.90727 0.00000
0.90752 0.00000
0.90777 0.00000
0.90802 0.00000
0.90827 0.00000
0.90852 0.00000
0.90877 0.00000
0.90902 0.00000
0.90927 0.00000
0.90952 0.00000
0.90977 0.00000
0.91003 0.00000
0.91028 0.00000
0.91053 0.00000
0.91078 0.00000
0.91103 0.00000
0.91128 0.00000
0.91153 0.00000
0.91178 0.00000
0.91203 0.00000
0.91228 0.00000
0.91253 0.00000
0.91278 0.00000
0.91303 0.00000
0.91328 0.00000
0.91353 0.00000
0.91378 0.00000
0.91404 0.00000
0.91429 0.00000
0.91454 0.00000
0.91479 0.00000
0.91504 0.00000
0.91529 0.00000
0.91554 0.00000
0.91579 0.00000
0.91604 0.00000
0.91629 0.00000
0.91654 0.00000
0.91679 0.00000
0.91704 0.00000
0.91729 0.00000
0.91754 0.00000
0.91779 0.00000
0.91805 0.00000
0.91830 0.00000
0.91855 0.00000
0.91880 0.00000
0.91905 0.00000
0.91930 0.00000
0.91955 0.00000
0.91980 0.00000
0.92005 0.00000
0.92030 0.00000
0.92055 0.00000
0.92080 0.00000
0.92105 0.00000
0.92130 0.00000
0.92155 0.00000
0.92180 0.00000
0.92206 0.00000
0.92231 0.00000
0.92256 0.00000
0.92281 0.00000
0.92306 0.00000
0.92331 0.00000
0.92356 0.00000
0.92381 0.00000
0.92406 0.00000
0.92431 0.00000
0.92456 0.00000
0.92481 0.00000
0.92506 0.00000
0.92531 0.00000
0.92556 0.00000
0.92581 0.00000
0.92607 0.00000
0.92632 0.00000
0.92657 0.00000
0.92682 0.00000
0.92707 0.00000
0.92732 0.00000
0.92757 0.00000
0.92782 0.00000
0.92807 0.00000
0.92832 0.00000
0.92857 0.00000
0.92882 0.00000
0.92907 0.00000
0.92932 0.00000
0.92957 0.00000
0.92982 0.00000
0.93008 0.00000
0.93033 0.00000
0.93058 0.00000
0.93083 0.00000
0.93108 0.00000
0.93133 0.00000
0.93158 0.00000
0.93183 0.00000
0.93208 0.00000
0.93233 0.00000
0.93258 0.00000
0.93283 0.00000
0.93308 0.00000
0.93333 0.00000
0.93358 0.00000
0.93383 0.00000
0.93409 0.00000
0.93434 0.00000
0.93459 0.00000
0.93484 0.00000
0.93509 0.00000
0.93534 0.00000
0.93559 0.00000
0.93584 0.00000
0.93609 0.00000
0.93634 0.00000
0.93659 0.00000
0.93684 0.00000
0.93709 0.00000
0.93734 0.00000
0.93759 0.00000
0.93784 0.00000
0.93810 0.00000
0.93835 0.00000
0.93860 0.00000
0.93885 0.00000
0.93910 0.00000
0.93935 0.00000
0.93960 0.00000
0.93985 0.00000
0.94010 0.00000
0.94035 0.00000
0.94060 0.00000
0.94085 0.00000
0.94110 0.00000
0.94135 0.00000
0.94160 0.00000
0.94185 0.00000
0.94211 0.00000
0.94236 0.00000
0.94261 0.00000
0.94286 0.00000
0.94311 0.00000
0.94336 0.00000
0.94361 0.00000
0.94386 0.00000
0.94411 0.00000
0.94436 0.00000
0.94461 0.00000
0.94486 0.00000
0.94511 0.00001
0.94536 0.00001
0.94561 0.00001
0.94586 0.00001
0.94612 0.00002
0.94637 0.00002
0.94662 0.00003
0.94687 0.00003
0.94712 0.00004
0.94737 0.00005
0.94762 0.00007
0.94787 0.00009
0.94812 0.00011
0.94837 0.00014
0.94862 0.00018
0.94887 0.00023
0.94912 0.00029
0.94937 0.00037
0.94962 0.00046
0.94987 0.00058
0.95013 0.00074
0.95038 0.00093
0.95063 0.00116
0.95088 0.00146
0.95113 0.00183
0.95138 0.00229
0.95163 0.00286
0.95188 0.00357
0.95213 0.00444
0.95238 0.00552
0.95263 0.00685
0.95288 0.00848
0.95313 0.01049
0.95338 0.01295
0.95363 0.01595
0.95388 0.01962
0.95414 0.02410
0.95439 0.02953
0.95464 0.03613
0.95489 0.04412
0.95514 0.05378
0.95539 0.06542
0.95564 0.07944
0.95589 0.09628
0.95614 0.11646
0.95639 0.14059
0.95664 0.16939
0.95689 0.20368
0.95714 0.24441
0.95739 0.29268
0.95764 0.34977
0.95789 0.41712
0.95815 0.49638
0.95840 0.58945
0.95865 0.69845
0.95890 0.82579
0.95915 0.97419
0.95940 1.14669
0.95965 1.34667
0.95990 1.57791
0.96015 1.84457
0.96040 2.15124
0.96065 2.50295
0.96090 2.90516
0.96115 3.36381
0.96140 3.88528
0.96165 4.47642
0.96190 5.14450
0.96216 5.89720
0.96241 6.74256
0.96266 7.68891
0.96291 8.74486
0.96316 9.91911
0.96341 11.22045
0.96366 12.65756
0.96391 14.23887
0.96416 15.97244
0.96441 17.86572
0.96466 19.92538
0.96491 22.15708
0.96516 24.56522
0.96541 27.15270
0.96566 29.92068
0.96591 32.86829
0.96617 35.99243
0.96642 39.28745
0.96667 42.74500
0.96692 46.35378
0.96717 50.09939
0.96742 53.96421
0.96767 57.92733
0.96792 61.96450
0.96817 66.04827
0.96842 70.14802
0.96867 74.23026
0.96892 78.25885
0.96917 82.19544
0.96942 85.99990
0.96967 89.63089
0.96992 93.04648
0.97018 96.20483
0.97043 99.06493
0.97068 101.58745
0.97093 103.73544
0.97118 105.47526
0.97143 106.77726
0.97168 107.61662
0.97193 107.97396
0.97218 107.83599
0.97243 107.19594
0.97268 106.05396
0.97293 104.41726
0.97318 102.30021
0.97343 99.72418
0.97368 96.71723
0.97393 93.31367
0.97419 89.55342
0.97444 85.48121
0.97469 81.14572
0.97494 76.59855
0.97519 71.89315
0.97544 67.08373
0.97569 62.22411
0.97594 57.36666
0.97619 52.56125
0.97644 47.85434
0.97669 43.28812
0.97694 38.89990
0.97719 34.72155
0.97744 30.77919
0.97769 27.09299
0.97794 23.67722
0.97820 20.54038
0.97845 17.68550
0.97870 15.11062
0.97895 12.80930
0.97920 10.77126
0.97945 8.98300
0.97970 7.42855
0.97995 6.09009
0.98020 4.94867
0.98045 3.98475
0.98070 3.17878
0.98095 2.51167
0.98120 1.96516
0.98145 1.52214
0.98170 1.16685
0.98195 0.88503
0.98221 0.66397
0.98246 0.49257
0.98271 0.36121
0.98296 0.26175
0.98321 0.18737
0.98346 0.13245
0.98371 0.09242
0.98396 0.06363
0.98421 0.04321
0.98446 0.02892
0.98471 0.01908
0.98496 0.01240
0.98521 0.00793
0.98546 0.00499
0.98571 0.00309
0.98596 0.00188
0.98622 0.00112
0.98647 0.00066
0.98672 0.00038
0.98697 0.00021
0.98722 0.00012
0.98747 0.00006
0.98772 0.00003
0.98797 0.00002
0.98822 0.00001
0.98847 0.00000
0.98872 0.00000
0.98897 0.00000
0.98922 0.00000
0.98947 0.00000
0.98972 0.00000
0.98997 0.00000
0.99023 0.00000
0.99048 0.00000
0.99073 0.00000
0.99098 0.00000
0.99123 0.00000
0.99148 0.00000
0.99173 0.00000
0.99198 0.00000
0.99223 0.00000
0.99248 0.00000
0.99273 0.00000
0.99298 0.00000
0.99323 0.00000
0.99348 0.00000
0.99373 0.00000
0.99398 0.00000
0.99424 0.00000
0.99449 0.00000
0.99474 0.00000
0.99499 0.00000
0.99524 0.00000
0.99549 0.00000
0.99574 0.00000
0.99599 0.00000
0.99624 0.00000
0.99649 0.00000
0.99674 0.00000
0.99699 0.00000
0.99724 0.00000
0.99749 0.00000
0.99774 0.00000
0.99799 0.00000
0.99825 0.00000
0.99850 0.00000
0.99875 0.00000
0.99900 0.00000
0.99925 0.00000
0.99950 0.00000
0.99975 0.00000
1.00000 0.00000


==> figures/fig_helpers/beta_coords_ncal2000_eps5_nq1_rho99.tex <==
0.65000 0.00000
0.65176 0.00000
0.65352 0.00000
0.65528 0.00000
0.65704 0.00000
0.65879 0.00000
0.66055 0.00000
0.66231 0.00000
0.66407 0.00000
0.66583 0.00000
0.66759 0.00000
0.66935 0.00000
0.67111 0.00000
0.67286 0.00000
0.67462 0.00000
0.67638 0.00000
0.67814 0.00000
0.67990 0.00000
0.68166 0.00000
0.68342 0.00000
0.68518 0.00000
0.68693 0.00000
0.68869 0.00000
0.69045 0.00000
0.69221 0.00000
0.69397 0.00000
0.69573 0.00000
0.69749 0.00000
0.69925 0.00000
0.70101 0.00000
0.70276 0.00000
0.70452 0.00000
0.70628 0.00000
0.70804 0.00000
0.70980 0.00000
0.71156 0.00000
0.71332 0.00000
0.71508 0.00000
0.71683 0.00000
0.71859 0.00000
0.72035 0.00000
0.72211 0.00000
0.72387 0.00000
0.72563 0.00000
0.72739 0.00000
0.72915 0.00000
0.73090 0.00000
0.73266 0.00000
0.73442 0.00000
0.73618 0.00000
0.73794 0.00000
0.73970 0.00000
0.74146 0.00000
0.74322 0.00000
0.74497 0.00000
0.74673 0.00000
0.74849 0.00000
0.75025 0.00000
0.75201 0.00000
0.75377 0.00000
0.75553 0.00000
0.75729 0.00000
0.75905 0.00000
0.76080 0.00000
0.76256 0.00000
0.76432 0.00000
0.76608 0.00000
0.76784 0.00000
0.76960 0.00000
0.77136 0.00000
0.77312 0.00000
0.77487 0.00000
0.77663 0.00000
0.77839 0.00000
0.78015 0.00000
0.78191 0.00000
0.78367 0.00000
0.78543 0.00000
0.78719 0.00000
0.78894 0.00000
0.79070 0.00000
0.79246 0.00000
0.79422 0.00000
0.79598 0.00000
0.79774 0.00000
0.79950 0.00000
0.80126 0.00000
0.80302 0.00000
0.80477 0.00000
0.80653 0.00000
0.80829 0.00000
0.81005 0.00000
0.81181 0.00000
0.81357 0.00000
0.81533 0.00000
0.81709 0.00000
0.81884 0.00000
0.82060 0.00000
0.82236 0.00000
0.82412 0.00000
0.82588 0.00000
0.82764 0.00000
0.82940 0.00000
0.83116 0.00000
0.83291 0.00000
0.83467 0.00000
0.83643 0.00000
0.83819 0.00000
0.83995 0.00000
0.84171 0.00000
0.84347 0.00000
0.84523 0.00000
0.84698 0.00000
0.84874 0.00000
0.85050 0.00000
0.85226 0.00000
0.85402 0.00000
0.85578 0.00000
0.85754 0.00000
0.85930 0.00000
0.86106 0.00000
0.86281 0.00000
0.86457 0.00000
0.86633 0.00000
0.86809 0.00000
0.86985 0.00000
0.87161 0.00000
0.87337 0.00000
0.87513 0.00000
0.87688 0.00000
0.87864 0.00000
0.88040 0.00000
0.88216 0.00000
0.88392 0.00000
0.88568 0.00000
0.88744 0.00000
0.88920 0.00000
0.89095 0.00000
0.89271 0.00000
0.89447 0.00000
0.89623 0.00000
0.89799 0.00000
0.89975 0.00000
0.90151 0.00000
0.90327 0.00000
0.90503 0.00000
0.90678 0.00000
0.90854 0.00000
0.91030 0.00000
0.91206 0.00000
0.91382 0.00000
0.91558 0.00000
0.91734 0.00000
0.91910 0.00002
0.92085 0.00009
0.92261 0.00036
0.92437 0.00137
0.92613 0.00496
0.92789 0.01677
0.92965 0.05315
0.93141 0.15725
0.93317 0.43298
0.93492 1.10566
0.93668 2.60882
0.93844 5.66458
0.94020 11.26888
0.94196 20.44074
0.94372 33.63074
0.94548 49.90020
0.94724 66.35130
0.94899 78.51502
0.95075 82.04792
0.95251 75.07284
0.95427 59.57527
0.95603 40.56923
0.95779 23.42542
0.95955 11.31583
0.96131 4.50360
0.96307 1.45126
0.96482 0.37117
0.96658 0.07363
0.96834 0.01103
0.97010 0.00121
0.97186 0.00009
0.97362 0.00000
0.97538 0.00000
0.97714 0.00000
0.97889 0.00000
0.98065 0.00000
0.98241 0.00000
0.98417 0.00000
0.98593 0.00000
0.98769 0.00000
0.98945 0.00000
0.99121 0.00000
0.99296 0.00000
0.99472 0.00000
0.99648 0.00000
0.99824 0.00000
1.00000 0.00000


==> figures/fig_helpers/beta_coords_ncal2000_eps5_nq3_rho18.tex <==
0.90000 0.00000
0.90025 0.00000
0.90050 0.00000
0.90075 0.00000
0.90100 0.00000
0.90125 0.00000
0.90150 0.00000
0.90175 0.00000
0.90201 0.00000
0.90226 0.00000
0.90251 0.00000
0.90276 0.00000
0.90301 0.00000
0.90326 0.00000
0.90351 0.00000
0.90376 0.00000
0.90401 0.00000
0.90426 0.00000
0.90451 0.00000
0.90476 0.00000
0.90501 0.00000
0.90526 0.00000
0.90551 0.00000
0.90576 0.00000
0.90602 0.00000
0.90627 0.00000
0.90652 0.00000
0.90677 0.00000
0.90702 0.00000
0.90727 0.00000
0.90752 0.00000
0.90777 0.00000
0.90802 0.00000
0.90827 0.00000
0.90852 0.00000
0.90877 0.00000
0.90902 0.00000
0.90927 0.00000
0.90952 0.00000
0.90977 0.00000
0.91003 0.00000
0.91028 0.00000
0.91053 0.00000
0.91078 0.00000
0.91103 0.00000
0.91128 0.00000
0.91153 0.00000
0.91178 0.00000
0.91203 0.00000
0.91228 0.00000
0.91253 0.00000
0.91278 0.00000
0.91303 0.00000
0.91328 0.00000
0.91353 0.00000
0.91378 0.00000
0.91404 0.00000
0.91429 0.00000
0.91454 0.00000
0.91479 0.00000
0.91504 0.00000
0.91529 0.00000
0.91554 0.00000
0.91579 0.00000
0.91604 0.00000
0.91629 0.00000
0.91654 0.00000
0.91679 0.00000
0.91704 0.00000
0.91729 0.00000
0.91754 0.00000
0.91779 0.00000
0.91805 0.00000
0.91830 0.00000
0.91855 0.00000
0.91880 0.00000
0.91905 0.00000
0.91930 0.00000
0.91955 0.00000
0.91980 0.00000
0.92005 0.00000
0.92030 0.00000
0.92055 0.00000
0.92080 0.00000
0.92105 0.00000
0.92130 0.00000
0.92155 0.00000
0.92180 0.00000
0.92206 0.00000
0.92231 0.00000
0.92256 0.00000
0.92281 0.00000
0.92306 0.00000
0.92331 0.00000
0.92356 0.00000
0.92381 0.00000
0.92406 0.00000
0.92431 0.00000
0.92456 0.00000
0.92481 0.00000
0.92506 0.00000
0.92531 0.00000
0.92556 0.00000
0.92581 0.00000
0.92607 0.00000
0.92632 0.00000
0.92657 0.00000
0.92682 0.00000
0.92707 0.00000
0.92732 0.00000
0.92757 0.00000
0.92782 0.00000
0.92807 0.00000
0.92832 0.00000
0.92857 0.00000
0.92882 0.00000
0.92907 0.00000
0.92932 0.00000
0.92957 0.00000
0.92982 0.00000
0.93008 0.00000
0.93033 0.00000
0.93058 0.00000
0.93083 0.00000
0.93108 0.00000
0.93133 0.00000
0.93158 0.00000
0.93183 0.00000
0.93208 0.00000
0.93233 0.00000
0.93258 0.00000
0.93283 0.00000
0.93308 0.00000
0.93333 0.00000
0.93358 0.00000
0.93383 0.00000
0.93409 0.00000
0.93434 0.00000
0.93459 0.00000
0.93484 0.00000
0.93509 0.00000
0.93534 0.00000
0.93559 0.00000
0.93584 0.00000
0.93609 0.00000
0.93634 0.00000
0.93659 0.00000
0.93684 0.00000
0.93709 0.00000
0.93734 0.00000
0.93759 0.00000
0.93784 0.00000
0.93810 0.00000
0.93835 0.00000
0.93860 0.00000
0.93885 0.00000
0.93910 0.00000
0.93935 0.00000
0.93960 0.00000
0.93985 0.00000
0.94010 0.00000
0.94035 0.00000
0.94060 0.00000
0.94085 0.00000
0.94110 0.00000
0.94135 0.00000
0.94160 0.00000
0.94185 0.00000
0.94211 0.00000
0.94236 0.00000
0.94261 0.00000
0.94286 0.00000
0.94311 0.00000
0.94336 0.00000
0.94361 0.00000
0.94386 0.00000
0.94411 0.00000
0.94436 0.00000
0.94461 0.00000
0.94486 0.00000
0.94511 0.00001
0.94536 0.00001
0.94561 0.00001
0.94586 0.00001
0.94612 0.00002
0.94637 0.00002
0.94662 0.00003
0.94687 0.00003
0.94712 0.00004
0.94737 0.00005
0.94762 0.00007
0.94787 0.00009
0.94812 0.00011
0.94837 0.00014
0.94862 0.00018
0.94887 0.00023
0.94912 0.00029
0.94937 0.00037
0.94962 0.00046
0.94987 0.00058
0.95013 0.00074
0.95038 0.00093
0.95063 0.00116
0.95088 0.00146
0.95113 0.00183
0.95138 0.00229
0.95163 0.00286
0.95188 0.00357
0.95213 0.00444
0.95238 0.00552
0.95263 0.00685
0.95288 0.00848
0.95313 0.01049
0.95338 0.01295
0.95363 0.01595
0.95388 0.01962
0.95414 0.02410
0.95439 0.02953
0.95464 0.03613
0.95489 0.04412
0.95514 0.05378
0.95539 0.06542
0.95564 0.07944
0.95589 0.09628
0.95614 0.11646
0.95639 0.14059
0.95664 0.16939
0.95689 0.20368
0.95714 0.24441
0.95739 0.29268
0.95764 0.34977
0.95789 0.41712
0.95815 0.49638
0.95840 0.58945
0.95865 0.69845
0.95890 0.82579
0.95915 0.97419
0.95940 1.14669
0.95965 1.34667
0.95990 1.57791
0.96015 1.84457
0.96040 2.15124
0.96065 2.50295
0.96090 2.90516
0.96115 3.36381
0.96140 3.88528
0.96165 4.47642
0.96190 5.14450
0.96216 5.89720
0.96241 6.74256
0.96266 7.68891
0.96291 8.74486
0.96316 9.91911
0.96341 11.22045
0.96366 12.65756
0.96391 14.23887
0.96416 15.97244
0.96441 17.86572
0.96466 19.92538
0.96491 22.15708
0.96516 24.56522
0.96541 27.15270
0.96566 29.92068
0.96591 32.86829
0.96617 35.99243
0.96642 39.28745
0.96667 42.74500
0.96692 46.35378
0.96717 50.09939
0.96742 53.96421
0.96767 57.92733
0.96792 61.96450
0.96817 66.04827
0.96842 70.14802
0.96867 74.23026
0.96892 78.25885
0.96917 82.19544
0.96942 85.99990
0.96967 89.63089
0.96992 93.04648
0.97018 96.20483
0.97043 99.06493
0.97068 101.58745
0.97093 103.73544
0.97118 105.47526
0.97143 106.77726
0.97168 107.61662
0.97193 107.97396
0.97218 107.83599
0.97243 107.19594
0.97268 106.05396
0.97293 104.41726
0.97318 102.30021
0.97343 99.72418
0.97368 96.71723
0.97393 93.31367
0.97419 89.55342
0.97444 85.48121
0.97469 81.14572
0.97494 76.59855
0.97519 71.89315
0.97544 67.08373
0.97569 62.22411
0.97594 57.36666
0.97619 52.56125
0.97644 47.85434
0.97669 43.28812
0.97694 38.89990
0.97719 34.72155
0.97744 30.77919
0.97769 27.09299
0.97794 23.67722
0.97820 20.54038
0.97845 17.68550
0.97870 15.11062
0.97895 12.80930
0.97920 10.77126
0.97945 8.98300
0.97970 7.42855
0.97995 6.09009
0.98020 4.94867
0.98045 3.98475
0.98070 3.17878
0.98095 2.51167
0.98120 1.96516
0.98145 1.52214
0.98170 1.16685
0.98195 0.88503
0.98221 0.66397
0.98246 0.49257
0.98271 0.36121
0.98296 0.26175
0.98321 0.18737
0.98346 0.13245
0.98371 0.09242
0.98396 0.06363
0.98421 0.04321
0.98446 0.02892
0.98471 0.01908
0.98496 0.01240
0.98521 0.00793
0.98546 0.00499
0.98571 0.00309
0.98596 0.00188
0.98622 0.00112
0.98647 0.00066
0.98672 0.00038
0.98697 0.00021
0.98722 0.00012
0.98747 0.00006
0.98772 0.00003
0.98797 0.00002
0.98822 0.00001
0.98847 0.00000
0.98872 0.00000
0.98897 0.00000
0.98922 0.00000
0.98947 0.00000
0.98972 0.00000
0.98997 0.00000
0.99023 0.00000
0.99048 0.00000
0.99073 0.00000
0.99098 0.00000
0.99123 0.00000
0.99148 0.00000
0.99173 0.00000
0.99198 0.00000
0.99223 0.00000
0.99248 0.00000
0.99273 0.00000
0.99298 0.00000
0.99323 0.00000
0.99348 0.00000
0.99373 0.00000
0.99398 0.00000
0.99424 0.00000
0.99449 0.00000
0.99474 0.00000
0.99499 0.00000
0.99524 0.00000
0.99549 0.00000
0.99574 0.00000
0.99599 0.00000
0.99624 0.00000
0.99649 0.00000
0.99674 0.00000
0.99699 0.00000
0.99724 0.00000
0.99749 0.00000
0.99774 0.00000
0.99799 0.00000
0.99825 0.00000
0.99850 0.00000
0.99875 0.00000
0.99900 0.00000
0.99925 0.00000
0.99950 0.00000
0.99975 0.00000
1.00000 0.00000


==> figures/fig_helpers/beta_coords_ncal2000_eps5_nq3_rho25.tex <==
0.90000 0.00000
0.90025 0.00000
0.90050 0.00000
0.90075 0.00000
0.90100 0.00000
0.90125 0.00000
0.90150 0.00000
0.90175 0.00000
0.90200 0.00000
0.90225 0.00000
0.90250 0.00000
0.90275 0.00000
0.90300 0.00000
0.90325 0.00000
0.90350 0.00000
0.90375 0.00000
0.90400 0.00000
0.90425 0.00000
0.90450 0.00000
0.90475 0.00000
0.90500 0.00000
0.90525 0.00000
0.90550 0.00000
0.90575 0.00000
0.90600 0.00000
0.90625 0.00000
0.90650 0.00000
0.90675 0.00000
0.90700 0.00000
0.90725 0.00000
0.90750 0.00000
0.90775 0.00000
0.90800 0.00000
0.90825 0.00000
0.90850 0.00000
0.90875 0.00000
0.90900 0.00000
0.90925 0.00000
0.90950 0.00000
0.90975 0.00000
0.91000 0.00000
0.91025 0.00000
0.91050 0.00000
0.91075 0.00000
0.91100 0.00000
0.91125 0.00000
0.91150 0.00000
0.91175 0.00000
0.91200 0.00000
0.91225 0.00000
0.91250 0.00000
0.91275 0.00000
0.91300 0.00000
0.91325 0.00000
0.91350 0.00000
0.91375 0.00000
0.91400 0.00000
0.91425 0.00000
0.91450 0.00000
0.91475 0.00000
0.91500 0.00000
0.91525 0.00000
0.91550 0.00000
0.91575 0.00000
0.91600 0.00000
0.91625 0.00000
0.91650 0.00000
0.91675 0.00000
0.91700 0.00000
0.91725 0.00000
0.91750 0.00000
0.91775 0.00000
0.91800 0.00000
0.91825 0.00000
0.91850 0.00000
0.91875 0.00000
0.91900 0.00000
0.91925 0.00000
0.91950 0.00000
0.91975 0.00000
0.92000 0.00000
0.92025 0.00000
0.92050 0.00000
0.92075 0.00000
0.92100 0.00000
0.92125 0.00000
0.92150 0.00000
0.92175 0.00000
0.92200 0.00000
0.92225 0.00000
0.92250 0.00000
0.92275 0.00000
0.92300 0.00000
0.92325 0.00000
0.92350 0.00000
0.92375 0.00000
0.92400 0.00000
0.92425 0.00000
0.92450 0.00000
0.92475 0.00000
0.92500 0.00000
0.92525 0.00000
0.92550 0.00000
0.92575 0.00000
0.92600 0.00000
0.92625 0.00000
0.92650 0.00000
0.92675 0.00000
0.92700 0.00000
0.92725 0.00000
0.92750 0.00000
0.92775 0.00000
0.92800 0.00000
0.92825 0.00000
0.92850 0.00000
0.92875 0.00000
0.92900 0.00000
0.92925 0.00000
0.92950 0.00000
0.92975 0.00000
0.93000 0.00000
0.93025 0.00000
0.93050 0.00000
0.93075 0.00000
0.93100 0.00000
0.93125 0.00000
0.93150 0.00001
0.93175 0.00001
0.93200 0.00001
0.93225 0.00001
0.93250 0.00002
0.93275 0.00002
0.93300 0.00002
0.93325 0.00003
0.93350 0.00004
0.93375 0.00005
0.93400 0.00006
0.93425 0.00007
0.93450 0.00009
0.93475 0.00011
0.93500 0.00014
0.93525 0.00018
0.93550 0.00022
0.93575 0.00027
0.93600 0.00034
0.93625 0.00041
0.93650 0.00051
0.93675 0.00063
0.93700 0.00078
0.93725 0.00096
0.93750 0.00117
0.93775 0.00144
0.93800 0.00176
0.93825 0.00215
0.93850 0.00263
0.93875 0.00321
0.93900 0.00390
0.93925 0.00475
0.93950 0.00576
0.93975 0.00698
0.94000 0.00846
0.94025 0.01022
0.94050 0.01234
0.94075 0.01487
0.94100 0.01789
0.94125 0.02149
0.94150 0.02579
0.94175 0.03089
0.94200 0.03694
0.94225 0.04411
0.94250 0.05259
0.94275 0.06260
0.94300 0.07440
0.94325 0.08828
0.94350 0.10457
0.94375 0.12367
0.94400 0.14601
0.94425 0.17211
0.94450 0.20252
0.94475 0.23791
0.94500 0.27900
0.94525 0.32662
0.94550 0.38171
0.94575 0.44531
0.94600 0.51859
0.94625 0.60285
0.94650 0.69954
0.94675 0.81026
0.94700 0.93679
0.94725 1.08108
0.94750 1.24527
0.94775 1.43171
0.94800 1.64294
0.94825 1.88173
0.94850 2.15107
0.94875 2.45418
0.94900 2.79450
0.94925 3.17571
0.94950 3.60170
0.94975 4.07658
0.95000 4.60469
0.95025 5.19051
0.95050 5.83872
0.95075 6.55412
0.95100 7.34163
0.95125 8.20619
0.95150 9.15280
0.95175 10.18638
0.95200 11.31177
0.95225 12.53362
0.95250 13.85633
0.95275 15.28397
0.95300 16.82018
0.95325 18.46806
0.95350 20.23011
0.95375 22.10809
0.95400 24.10292
0.95425 26.21460
0.95450 28.44204
0.95475 30.78304
0.95500 33.23413
0.95525 35.79049
0.95550 38.44592
0.95575 41.19269
0.95600 44.02157
0.95625 46.92176
0.95650 49.88087
0.95675 52.88496
0.95700 55.91856
0.95725 58.96475
0.95750 62.00523
0.95775 65.02049
0.95800 67.98989
0.95825 70.89192
0.95850 73.70437
0.95875 76.40458
0.95900 78.96969
0.95925 81.37696
0.95950 83.60400
0.95975 85.62918
0.96000 87.43186
0.96025 88.99278
0.96050 90.29433
0.96075 91.32086
0.96100 92.05902
0.96125 92.49793
0.96150 92.62950
0.96175 92.44855
0.96200 91.95300
0.96225 91.14396
0.96250 90.02578
0.96275 88.60603
0.96300 86.89546
0.96325 84.90787
0.96350 82.65992
0.96375 80.17094
0.96400 77.46263
0.96425 74.55875
0.96450 71.48478
0.96475 68.26749
0.96500 64.93460
0.96525 61.51431
0.96550 58.03492
0.96575 54.52436
0.96600 51.00985
0.96625 47.51751
0.96650 44.07197
0.96675 40.69611
0.96700 37.41081
0.96725 34.23467
0.96750 31.18392
0.96775 28.27228
0.96800 25.51089
0.96825 22.90834
0.96850 20.47069
0.96875 18.20159
0.96900 16.10239
0.96925 14.17232
0.96950 12.40868
0.96975 10.80706
0.97000 9.36161
0.97025 8.06520
0.97050 6.90976
0.97075 5.88645
0.97100 4.98593
0.97125 4.19854
0.97150 3.51452
0.97175 2.92419
0.97200 2.41808
0.97225 1.98707
0.97250 1.62251
0.97275 1.31627
0.97300 1.06079
0.97325 0.84917
0.97350 0.67512
0.97375 0.53301
0.97400 0.41783
0.97425 0.32518
0.97450 0.25121
0.97475 0.19261
0.97500 0.14655
0.97525 0.11064
0.97550 0.08286
0.97575 0.06155
0.97600 0.04535
0.97625 0.03313
0.97650 0.02399
0.97675 0.01722
0.97700 0.01225
0.97725 0.00863
0.97750 0.00603
0.97775 0.00417
0.97800 0.00285
0.97825 0.00194
0.97850 0.00130
0.97875 0.00086
0.97900 0.00057
0.97925 0.00037
0.97950 0.00024
0.97975 0.00015
0.98000 0.00009
0.98025 0.00006
0.98050 0.00004
0.98075 0.00002
0.98100 0.00001
0.98125 0.00001
0.98150 0.00000
0.98175 0.00000
0.98200 0.00000
0.98225 0.00000
0.98250 0.00000
0.98275 0.00000
0.98300 0.00000
0.98325 0.00000
0.98350 0.00000
0.98375 0.00000
0.98400 0.00000
0.98425 0.00000
0.98450 0.00000
0.98475 0.00000
0.98500 0.00000
0.98525 0.00000
0.98550 0.00000
0.98575 0.00000
0.98600 0.00000
0.98625 0.00000
0.98650 0.00000
0.98675 0.00000
0.98700 0.00000
0.98725 0.00000
0.98750 0.00000
0.98775 0.00000
0.98800 0.00000
0.98825 0.00000
0.98850 0.00000
0.98875 0.00000
0.98900 0.00000
0.98925 0.00000
0.98950 0.00000
0.98975 0.00000
0.99000 0.00000
0.99025 0.00000
0.99050 0.00000
0.99075 0.00000
0.99100 0.00000
0.99125 0.00000
0.99150 0.00000
0.99175 0.00000
0.99200 0.00000
0.99225 0.00000
0.99250 0.00000
0.99275 0.00000
0.99300 0.00000
0.99325 0.00000
0.99350 0.00000
0.99375 0.00000
0.99400 0.00000
0.99425 0.00000
0.99450 0.00000
0.99475 0.00000
0.99500 0.00000
0.99525 0.00000
0.99550 0.00000
0.99575 0.00000
0.99600 0.00000
0.99625 0.00000
0.99650 0.00000
0.99675 0.00000
0.99700 0.00000
0.99725 0.00000
0.99750 0.00000
0.99775 0.00000
0.99800 0.00000
0.99825 0.00000
0.99850 0.00000
0.99875 0.00000
0.99900 0.00000
0.99925 0.00000
0.99950 0.00000
0.99975 0.00000
1.00000 0.00000


==> figures/fig_helpers/beta_coords_ncal2000_eps5_nq3_rho32.tex <==
0.65000 0.00000
0.65176 0.00000
0.65352 0.00000
0.65528 0.00000
0.65704 0.00000
0.65879 0.00000
0.66055 0.00000
0.66231 0.00000
0.66407 0.00000
0.66583 0.00000
0.66759 0.00000
0.66935 0.00000
0.67111 0.00000
0.67286 0.00000
0.67462 0.00000
0.67638 0.00000
0.67814 0.00000
0.67990 0.00000
0.68166 0.00000
0.68342 0.00000
0.68518 0.00000
0.68693 0.00000
0.68869 0.00000
0.69045 0.00000
0.69221 0.00000
0.69397 0.00000
0.69573 0.00000
0.69749 0.00000
0.69925 0.00000
0.70101 0.00000
0.70276 0.00000
0.70452 0.00000
0.70628 0.00000
0.70804 0.00000
0.70980 0.00000
0.71156 0.00000
0.71332 0.00000
0.71508 0.00000
0.71683 0.00000
0.71859 0.00000
0.72035 0.00000
0.72211 0.00000
0.72387 0.00000
0.72563 0.00000
0.72739 0.00000
0.72915 0.00000
0.73090 0.00000
0.73266 0.00000
0.73442 0.00000
0.73618 0.00000
0.73794 0.00000
0.73970 0.00000
0.74146 0.00000
0.74322 0.00000
0.74497 0.00000
0.74673 0.00000
0.74849 0.00000
0.75025 0.00000
0.75201 0.00000
0.75377 0.00000
0.75553 0.00000
0.75729 0.00000
0.75905 0.00000
0.76080 0.00000
0.76256 0.00000
0.76432 0.00000
0.76608 0.00000
0.76784 0.00000
0.76960 0.00000
0.77136 0.00000
0.77312 0.00000
0.77487 0.00000
0.77663 0.00000
0.77839 0.00000
0.78015 0.00000
0.78191 0.00000
0.78367 0.00000
0.78543 0.00000
0.78719 0.00000
0.78894 0.00000
0.79070 0.00000
0.79246 0.00000
0.79422 0.00000
0.79598 0.00000
0.79774 0.00000
0.79950 0.00000
0.80126 0.00000
0.80302 0.00000
0.80477 0.00000
0.80653 0.00000
0.80829 0.00000
0.81005 0.00000
0.81181 0.00000
0.81357 0.00000
0.81533 0.00000
0.81709 0.00000
0.81884 0.00000
0.82060 0.00000
0.82236 0.00000
0.82412 0.00000
0.82588 0.00000
0.82764 0.00000
0.82940 0.00000
0.83116 0.00000
0.83291 0.00000
0.83467 0.00000
0.83643 0.00000
0.83819 0.00000
0.83995 0.00000
0.84171 0.00000
0.84347 0.00000
0.84523 0.00000
0.84698 0.00000
0.84874 0.00000
0.85050 0.00000
0.85226 0.00000
0.85402 0.00000
0.85578 0.00000
0.85754 0.00000
0.85930 0.00000
0.86106 0.00000
0.86281 0.00000
0.86457 0.00000
0.86633 0.00000
0.86809 0.00000
0.86985 0.00000
0.87161 0.00000
0.87337 0.00000
0.87513 0.00000
0.87688 0.00000
0.87864 0.00000
0.88040 0.00000
0.88216 0.00000
0.88392 0.00000
0.88568 0.00000
0.88744 0.00000
0.88920 0.00000
0.89095 0.00000
0.89271 0.00000
0.89447 0.00000
0.89623 0.00000
0.89799 0.00000
0.89975 0.00000
0.90151 0.00000
0.90327 0.00000
0.90503 0.00000
0.90678 0.00000
0.90854 0.00000
0.91030 0.00000
0.91206 0.00000
0.91382 0.00000
0.91558 0.00000
0.91734 0.00000
0.91910 0.00001
0.92085 0.00005
0.92261 0.00022
0.92437 0.00088
0.92613 0.00324
0.92789 0.01124
0.92965 0.03658
0.93141 0.11120
0.93317 0.31483
0.93492 0.82725
0.93668 2.00989
0.93844 4.49723
0.94020 9.22700
0.94196 17.27640
0.94372 29.36751
0.94548 45.06401
0.94724 62.03325
0.94899 76.07760
0.95075 82.49274
0.95251 78.42020
0.95427 64.74447
0.95603 45.93740
0.95779 27.68115
0.95955 13.97859
0.96131 5.82690
0.96307 1.97070
0.96482 0.53019
0.96658 0.11091
0.96834 0.01757
0.97010 0.00204
0.97186 0.00017
0.97362 0.00001
0.97538 0.00000
0.97714 0.00000
0.97889 0.00000
0.98065 0.00000
0.98241 0.00000
0.98417 0.00000
0.98593 0.00000
0.98769 0.00000
0.98945 0.00000
0.99121 0.00000
0.99296 0.00000
0.99472 0.00000
0.99648 0.00000
0.99824 0.00000
1.00000 0.00000


==> figures/fig_helpers/beta_coords_ncal500_eps5_nq1_rho13.tex <==
0.90000 0.00000
0.90025 0.00000
0.90050 0.00000
0.90075 0.00000
0.90100 0.00000
0.90125 0.00000
0.90150 0.00000
0.90175 0.00000
0.90200 0.00000
0.90225 0.00000
0.90250 0.00000
0.90275 0.00000
0.90300 0.00000
0.90325 0.00000
0.90350 0.00000
0.90375 0.00000
0.90400 0.00000
0.90425 0.00000
0.90450 0.00000
0.90475 0.00000
0.90500 0.00000
0.90525 0.00000
0.90550 0.00000
0.90575 0.00000
0.90600 0.00000
0.90625 0.00000
0.90650 0.00000
0.90675 0.00000
0.90700 0.00000
0.90725 0.00000
0.90750 0.00000
0.90775 0.00000
0.90800 0.00000
0.90825 0.00000
0.90850 0.00000
0.90875 0.00000
0.90900 0.00000
0.90925 0.00000
0.90950 0.00000
0.90975 0.00000
0.91000 0.00000
0.91025 0.00000
0.91050 0.00000
0.91075 0.00000
0.91100 0.00000
0.91125 0.00000
0.91150 0.00000
0.91175 0.00001
0.91200 0.00001
0.91225 0.00001
0.91250 0.00001
0.91275 0.00001
0.91300 0.00001
0.91325 0.00001
0.91350 0.00001
0.91375 0.00001
0.91400 0.00001
0.91425 0.00001
0.91450 0.00001
0.91475 0.00002
0.91500 0.00002
0.91525 0.00002
0.91550 0.00002
0.91575 0.00002
0.91600 0.00003
0.91625 0.00003
0.91650 0.00003
0.91675 0.00003
0.91700 0.00004
0.91725 0.00004
0.91750 0.00004
0.91775 0.00005
0.91800 0.00005
0.91825 0.00006
0.91850 0.00007
0.91875 0.00007
0.91900 0.00008
0.91925 0.00009
0.91950 0.00009
0.91975 0.00010
0.92000 0.00011
0.92025 0.00012
0.92050 0.00014
0.92075 0.00015
0.92100 0.00016
0.92125 0.00018
0.92150 0.00019
0.92175 0.00021
0.92200 0.00023
0.92225 0.00026
0.92250 0.00028
0.92275 0.00031
0.92300 0.00033
0.92325 0.00037
0.92350 0.00040
0.92375 0.00044
0.92400 0.00048
0.92425 0.00052
0.92450 0.00057
0.92475 0.00062
0.92500 0.00068
0.92525 0.00074
0.92550 0.00081
0.92575 0.00088
0.92600 0.00096
0.92625 0.00105
0.92650 0.00115
0.92675 0.00125
0.92700 0.00137
0.92725 0.00149
0.92750 0.00162
0.92775 0.00177
0.92800 0.00193
0.92825 0.00210
0.92850 0.00229
0.92875 0.00249
0.92900 0.00271
0.92925 0.00295
0.92950 0.00322
0.92975 0.00350
0.93000 0.00381
0.93025 0.00414
0.93050 0.00450
0.93075 0.00490
0.93100 0.00532
0.93125 0.00578
0.93150 0.00629
0.93175 0.00683
0.93200 0.00742
0.93225 0.00806
0.93250 0.00875
0.93275 0.00949
0.93300 0.01030
0.93325 0.01118
0.93350 0.01213
0.93375 0.01315
0.93400 0.01426
0.93425 0.01546
0.93450 0.01676
0.93475 0.01816
0.93500 0.01967
0.93525 0.02131
0.93550 0.02307
0.93575 0.02498
0.93600 0.02704
0.93625 0.02926
0.93650 0.03165
0.93675 0.03423
0.93700 0.03702
0.93725 0.04002
0.93750 0.04325
0.93775 0.04674
0.93800 0.05049
0.93825 0.05453
0.93850 0.05888
0.93875 0.06356
0.93900 0.06860
0.93925 0.07401
0.93950 0.07984
0.93975 0.08609
0.94000 0.09282
0.94025 0.10004
0.94050 0.10780
0.94075 0.11613
0.94100 0.12507
0.94125 0.13467
0.94150 0.14496
0.94175 0.15599
0.94200 0.16782
0.94225 0.18049
0.94250 0.19407
0.94275 0.20861
0.94300 0.22418
0.94325 0.24084
0.94350 0.25866
0.94375 0.27772
0.94400 0.29811
0.94425 0.31989
0.94450 0.34316
0.94475 0.36802
0.94500 0.39456
0.94525 0.42288
0.94550 0.45310
0.94575 0.48533
0.94600 0.51969
0.94625 0.55632
0.94650 0.59533
0.94675 0.63688
0.94700 0.68110
0.94725 0.72817
0.94750 0.77823
0.94775 0.83146
0.94800 0.88804
0.94825 0.94815
0.94850 1.01199
0.94875 1.07976
0.94900 1.15167
0.94925 1.22795
0.94950 1.30882
0.94975 1.39453
0.95000 1.48532
0.95025 1.58145
0.95050 1.68320
0.95075 1.79084
0.95100 1.90466
0.95125 2.02496
0.95150 2.15205
0.95175 2.28625
0.95200 2.42790
0.95225 2.57732
0.95250 2.73487
0.95275 2.90091
0.95300 3.07581
0.95325 3.25994
0.95350 3.45370
0.95375 3.65748
0.95400 3.87168
0.95425 4.09671
0.95450 4.33300
0.95475 4.58096
0.95500 4.84104
0.95525 5.11365
0.95550 5.39925
0.95575 5.69827
0.95600 6.01115
0.95625 6.33834
0.95650 6.68028
0.95675 7.03742
0.95700 7.41018
0.95725 7.79900
0.95750 8.20430
0.95775 8.62650
0.95800 9.06599
0.95825 9.52317
0.95850 9.99842
0.95875 10.49208
0.95900 11.00450
0.95925 11.53598
0.95950 12.08682
0.95975 12.65728
0.96000 13.24757
0.96025 13.85789
0.96050 14.48841
0.96075 15.13923
0.96100 15.81042
0.96125 16.50200
0.96150 17.21396
0.96175 17.94620
0.96200 18.69859
0.96225 19.47092
0.96250 20.26293
0.96275 21.07429
0.96300 21.90458
0.96325 22.75334
0.96350 23.61999
0.96375 24.50390
0.96400 25.40435
0.96425 26.32051
0.96450 27.25150
0.96475 28.19631
0.96500 29.15385
0.96525 30.12294
0.96550 31.10229
0.96575 32.09053
0.96600 33.08616
0.96625 34.08761
0.96650 35.09318
0.96675 36.10109
0.96700 37.10946
0.96725 38.11631
0.96750 39.11956
0.96775 40.11704
0.96800 41.10649
0.96825 42.08557
0.96850 43.05187
0.96875 44.00287
0.96900 44.93603
0.96925 45.84871
0.96950 46.73823
0.96975 47.60187
0.97000 48.43688
0.97025 49.24047
0.97050 50.00985
0.97075 50.74221
0.97100 51.43476
0.97125 52.08474
0.97150 52.68942
0.97175 53.24611
0.97200 53.75219
0.97225 54.20514
0.97250 54.60250
0.97275 54.94194
0.97300 55.22126
0.97325 55.43840
0.97350 55.59144
0.97375 55.67866
0.97400 55.69851
0.97425 55.64966
0.97450 55.53097
0.97475 55.34157
0.97500 55.08082
0.97525 54.74831
0.97550 54.34394
0.97575 53.86787
0.97600 53.32054
0.97625 52.70269
0.97650 52.01536
0.97675 51.25987
0.97700 50.43788
0.97725 49.55133
0.97750 48.60244
0.97775 47.59376
0.97800 46.52810
0.97825 45.40856
0.97850 44.23850
0.97875 43.02153
0.97900 41.76150
0.97925 40.46246
0.97950 39.12868
0.97975 37.76458
0.98000 36.37473
0.98025 34.96382
0.98050 33.53664
0.98075 32.09804
0.98100 30.65289
0.98125 29.20607
0.98150 27.76241
0.98175 26.32671
0.98200 24.90363
0.98225 23.49773
0.98250 22.11339
0.98275 20.75481
0.98300 19.42597
0.98325 18.13058
0.98350 16.87211
0.98375 15.65370
0.98400 14.47820
0.98425 13.34812
0.98450 12.26561
0.98475 11.23249
0.98500 10.25018
0.98525 9.31976
0.98550 8.44195
0.98575 7.61707
0.98600 6.84514
0.98625 6.12579
0.98650 5.45835
0.98675 4.84185
0.98700 4.27501
0.98725 3.75630
0.98750 3.28398
0.98775 2.85606
0.98800 2.47041
0.98825 2.12474
0.98850 1.81665
0.98875 1.54368
0.98900 1.30329
0.98925 1.09293
0.98950 0.91007
0.98975 0.75222
0.99000 0.61694
0.99025 0.50187
0.99050 0.40478
0.99075 0.32354
0.99100 0.25614
0.99125 0.20076
0.99150 0.15568
0.99175 0.11937
0.99200 0.09044
0.99225 0.06766
0.99250 0.04993
0.99275 0.03632
0.99300 0.02601
0.99325 0.01832
0.99350 0.01268
0.99375 0.00860
0.99400 0.00572
0.99425 0.00372
0.99450 0.00236
0.99475 0.00145
0.99500 0.00087
0.99525 0.00051
0.99550 0.00028
0.99575 0.00015
0.99600 0.00008
0.99625 0.00004
0.99650 0.00002
0.99675 0.00001
0.99700 0.00000
0.99725 0.00000
0.99750 0.00000
0.99775 0.00000
0.99800 0.00000
0.99825 0.00000
0.99850 0.00000
0.99875 0.00000
0.99900 0.00000
0.99925 0.00000
0.99950 0.00000
0.99975 0.00000
1.00000 0.00000


==> figures/fig_helpers/beta_coords_ncal500_eps5_nq1_rho24.tex <==
0.65000 0.00000
0.65176 0.00000
0.65352 0.00000
0.65528 0.00000
0.65704 0.00000
0.65879 0.00000
0.66055 0.00000
0.66231 0.00000
0.66407 0.00000
0.66583 0.00000
0.66759 0.00000
0.66935 0.00000
0.67111 0.00000
0.67286 0.00000
0.67462 0.00000
0.67638 0.00000
0.67814 0.00000
0.67990 0.00000
0.68166 0.00000
0.68342 0.00000
0.68518 0.00000
0.68693 0.00000
0.68869 0.00000
0.69045 0.00000
0.69221 0.00000
0.69397 0.00000
0.69573 0.00000
0.69749 0.00000
0.69925 0.00000
0.70101 0.00000
0.70276 0.00000
0.70452 0.00000
0.70628 0.00000
0.70804 0.00000
0.70980 0.00000
0.71156 0.00000
0.71332 0.00000
0.71508 0.00000
0.71683 0.00000
0.71859 0.00000
0.72035 0.00000
0.72211 0.00000
0.72387 0.00000
0.72563 0.00000
0.72739 0.00000
0.72915 0.00000
0.73090 0.00000
0.73266 0.00000
0.73442 0.00000
0.73618 0.00000
0.73794 0.00000
0.73970 0.00000
0.74146 0.00000
0.74322 0.00000
0.74497 0.00000
0.74673 0.00000
0.74849 0.00000
0.75025 0.00000
0.75201 0.00000
0.75377 0.00000
0.75553 0.00000
0.75729 0.00000
0.75905 0.00000
0.76080 0.00000
0.76256 0.00000
0.76432 0.00000
0.76608 0.00000
0.76784 0.00000
0.76960 0.00000
0.77136 0.00000
0.77312 0.00000
0.77487 0.00000
0.77663 0.00000
0.77839 0.00000
0.78015 0.00000
0.78191 0.00000
0.78367 0.00000
0.78543 0.00000
0.78719 0.00000
0.78894 0.00000
0.79070 0.00000
0.79246 0.00000
0.79422 0.00000
0.79598 0.00000
0.79774 0.00000
0.79950 0.00000
0.80126 0.00000
0.80302 0.00000
0.80477 0.00000
0.80653 0.00000
0.80829 0.00000
0.81005 0.00000
0.81181 0.00000
0.81357 0.00000
0.81533 0.00000
0.81709 0.00000
0.81884 0.00000
0.82060 0.00000
0.82236 0.00000
0.82412 0.00000
0.82588 0.00000
0.82764 0.00000
0.82940 0.00000
0.83116 0.00000
0.83291 0.00000
0.83467 0.00000
0.83643 0.00000
0.83819 0.00000
0.83995 0.00000
0.84171 0.00000
0.84347 0.00000
0.84523 0.00000
0.84698 0.00000
0.84874 0.00000
0.85050 0.00000
0.85226 0.00000
0.85402 0.00000
0.85578 0.00000
0.85754 0.00000
0.85930 0.00000
0.86106 0.00000
0.86281 0.00000
0.86457 0.00000
0.86633 0.00000
0.86809 0.00000
0.86985 0.00000
0.87161 0.00000
0.87337 0.00000
0.87513 0.00000
0.87688 0.00000
0.87864 0.00001
0.88040 0.00001
0.88216 0.00002
0.88392 0.00003
0.88568 0.00006
0.88744 0.00010
0.88920 0.00018
0.89095 0.00032
0.89271 0.00055
0.89447 0.00094
0.89623 0.00159
0.89799 0.00268
0.89975 0.00447
0.90151 0.00739
0.90327 0.01211
0.90503 0.01963
0.90678 0.03153
0.90854 0.05011
0.91030 0.07879
0.91206 0.12253
0.91382 0.18840
0.91558 0.28630
0.91734 0.42981
0.91910 0.63716
0.92085 0.93228
0.92261 1.34567
0.92437 1.91512
0.92613 2.68577
0.92789 3.70927
0.92965 5.04154
0.93141 6.73881
0.93317 8.85142
0.93492 11.41534
0.93668 14.44171
0.93844 17.90504
0.94020 21.73178
0.94196 25.79129
0.94372 29.89207
0.94548 33.78614
0.94724 37.18397
0.94899 39.78085
0.95075 41.29359
0.95251 41.50326
0.95427 40.29682
0.95603 37.69888
0.95779 33.88424
0.95955 29.16487
0.96131 23.95010
0.96307 18.68558
0.96482 13.78338
0.96658 9.55937
0.96834 6.19308
0.97010 3.71950
0.97186 2.05237
0.97362 1.02933
0.97538 0.46318
0.97714 0.18406
0.97889 0.06334
0.98065 0.01841
0.98241 0.00438
0.98417 0.00082
0.98593 0.00011
0.98769 0.00001
0.98945 0.00000
0.99121 0.00000
0.99296 0.00000
0.99472 0.00000
0.99648 0.00000
0.99824 0.00000
1.00000 0.00000


==> figures/fig_helpers/beta_coords_ncal500_eps5_nq1_rho5.tex <==
0.90000 0.00000
0.90025 0.00000
0.90050 0.00000
0.90075 0.00000
0.90100 0.00000
0.90125 0.00000
0.90150 0.00000
0.90175 0.00000
0.90201 0.00000
0.90226 0.00000
0.90251 0.00000
0.90276 0.00000
0.90301 0.00000
0.90326 0.00000
0.90351 0.00000
0.90376 0.00000
0.90401 0.00000
0.90426 0.00000
0.90451 0.00000
0.90476 0.00000
0.90501 0.00000
0.90526 0.00000
0.90551 0.00000
0.90576 0.00000
0.90602 0.00000
0.90627 0.00000
0.90652 0.00000
0.90677 0.00000
0.90702 0.00000
0.90727 0.00000
0.90752 0.00000
0.90777 0.00000
0.90802 0.00000
0.90827 0.00000
0.90852 0.00000
0.90877 0.00000
0.90902 0.00000
0.90927 0.00000
0.90952 0.00000
0.90977 0.00000
0.91003 0.00000
0.91028 0.00000
0.91053 0.00000
0.91078 0.00000
0.91103 0.00000
0.91128 0.00000
0.91153 0.00000
0.91178 0.00000
0.91203 0.00000
0.91228 0.00000
0.91253 0.00000
0.91278 0.00000
0.91303 0.00000
0.91328 0.00000
0.91353 0.00000
0.91378 0.00000
0.91404 0.00000
0.91429 0.00000
0.91454 0.00000
0.91479 0.00000
0.91504 0.00000
0.91529 0.00000
0.91554 0.00000
0.91579 0.00000
0.91604 0.00000
0.91629 0.00000
0.91654 0.00000
0.91679 0.00000
0.91704 0.00000
0.91729 0.00000
0.91754 0.00000
0.91779 0.00000
0.91805 0.00000
0.91830 0.00000
0.91855 0.00000
0.91880 0.00000
0.91905 0.00000
0.91930 0.00000
0.91955 0.00000
0.91980 0.00000
0.92005 0.00000
0.92030 0.00000
0.92055 0.00000
0.92080 0.00000
0.92105 0.00000
0.92130 0.00000
0.92155 0.00000
0.92180 0.00000
0.92206 0.00000
0.92231 0.00000
0.92256 0.00000
0.92281 0.00000
0.92306 0.00000
0.92331 0.00000
0.92356 0.00000
0.92381 0.00000
0.92406 0.00000
0.92431 0.00000
0.92456 0.00000
0.92481 0.00000
0.92506 0.00000
0.92531 0.00000
0.92556 0.00000
0.92581 0.00000
0.92607 0.00000
0.92632 0.00000
0.92657 0.00000
0.92682 0.00000
0.92707 0.00000
0.92732 0.00000
0.92757 0.00000
0.92782 0.00000
0.92807 0.00000
0.92832 0.00000
0.92857 0.00000
0.92882 0.00000
0.92907 0.00000
0.92932 0.00000
0.92957 0.00000
0.92982 0.00000
0.93008 0.00000
0.93033 0.00000
0.93058 0.00000
0.93083 0.00000
0.93108 0.00000
0.93133 0.00000
0.93158 0.00000
0.93183 0.00000
0.93208 0.00000
0.93233 0.00000
0.93258 0.00000
0.93283 0.00000
0.93308 0.00000
0.93333 0.00000
0.93358 0.00000
0.93383 0.00000
0.93409 0.00000
0.93434 0.00000
0.93459 0.00000
0.93484 0.00000
0.93509 0.00000
0.93534 0.00000
0.93559 0.00000
0.93584 0.00000
0.93609 0.00000
0.93634 0.00000
0.93659 0.00000
0.93684 0.00000
0.93709 0.00000
0.93734 0.00000
0.93759 0.00000
0.93784 0.00000
0.93810 0.00000
0.93835 0.00000
0.93860 0.00000
0.93885 0.00000
0.93910 0.00000
0.93935 0.00000
0.93960 0.00000
0.93985 0.00000
0.94010 0.00001
0.94035 0.00001
0.94060 0.00001
0.94085 0.00001
0.94110 0.00001
0.94135 0.00001
0.94160 0.00001
0.94185 0.00001
0.94211 0.00001
0.94236 0.00001
0.94261 0.00002
0.94286 0.00002
0.94311 0.00002
0.94336 0.00002
0.94361 0.00003
0.94386 0.00003
0.94411 0.00003
0.94436 0.00004
0.94461 0.00004
0.94486 0.00004
0.94511 0.00005
0.94536 0.00005
0.94561 0.00006
0.94586 0.00007
0.94612 0.00008
0.94637 0.00008
0.94662 0.00009
0.94687 0.00010
0.94712 0.00012
0.94737 0.00013
0.94762 0.00014
0.94787 0.00016
0.94812 0.00018
0.94837 0.00020
0.94862 0.00022
0.94887 0.00024
0.94912 0.00027
0.94937 0.00030
0.94962 0.00033
0.94987 0.00037
0.95013 0.00041
0.95038 0.00046
0.95063 0.00051
0.95088 0.00056
0.95113 0.00063
0.95138 0.00070
0.95163 0.00077
0.95188 0.00086
0.95213 0.00095
0.95238 0.00105
0.95263 0.00117
0.95288 0.00130
0.95313 0.00144
0.95338 0.00159
0.95363 0.00177
0.95388 0.00196
0.95414 0.00217
0.95439 0.00240
0.95464 0.00266
0.95489 0.00295
0.95514 0.00326
0.95539 0.00361
0.95564 0.00400
0.95589 0.00442
0.95614 0.00489
0.95639 0.00541
0.95664 0.00599
0.95689 0.00662
0.95714 0.00731
0.95739 0.00808
0.95764 0.00893
0.95789 0.00987
0.95815 0.01090
0.95840 0.01204
0.95865 0.01329
0.95890 0.01467
0.95915 0.01618
0.95940 0.01786
0.95965 0.01970
0.95990 0.02172
0.96015 0.02395
0.96040 0.02640
0.96065 0.02909
0.96090 0.03205
0.96115 0.03531
0.96140 0.03888
0.96165 0.04280
0.96190 0.04712
0.96216 0.05185
0.96241 0.05704
0.96266 0.06273
0.96291 0.06898
0.96316 0.07583
0.96341 0.08334
0.96366 0.09156
0.96391 0.10057
0.96416 0.11044
0.96441 0.12124
0.96466 0.13306
0.96491 0.14599
0.96516 0.16013
0.96541 0.17559
0.96566 0.19249
0.96591 0.21094
0.96617 0.23110
0.96642 0.25311
0.96667 0.27712
0.96692 0.30332
0.96717 0.33188
0.96742 0.36302
0.96767 0.39695
0.96792 0.43391
0.96817 0.47415
0.96842 0.51794
0.96867 0.56557
0.96892 0.61738
0.96917 0.67368
0.96942 0.73485
0.96967 0.80128
0.96992 0.87339
0.97018 0.95163
0.97043 1.03648
0.97068 1.12844
0.97093 1.22808
0.97118 1.33598
0.97143 1.45276
0.97168 1.57908
0.97193 1.71567
0.97218 1.86326
0.97243 2.02266
0.97268 2.19472
0.97293 2.38033
0.97318 2.58046
0.97343 2.79609
0.97368 3.02830
0.97393 3.27820
0.97419 3.54696
0.97444 3.83582
0.97469 4.14608
0.97494 4.47909
0.97519 4.83627
0.97544 5.21911
0.97569 5.62913
0.97594 6.06794
0.97619 6.53719
0.97644 7.03861
0.97669 7.57395
0.97694 8.14503
0.97719 8.75371
0.97744 9.40189
0.97769 10.09152
0.97794 10.82454
0.97820 11.60293
0.97845 12.42868
0.97870 13.30376
0.97895 14.23015
0.97920 15.20977
0.97945 16.24450
0.97970 17.33617
0.97995 18.48652
0.98020 19.69715
0.98045 20.96959
0.98070 22.30517
0.98095 23.70504
0.98120 25.17015
0.98145 26.70122
0.98170 28.29864
0.98195 29.96254
0.98221 31.69267
0.98246 33.48839
0.98271 35.34862
0.98296 37.27182
0.98321 39.25592
0.98346 41.29828
0.98371 43.39566
0.98396 45.54416
0.98421 47.73918
0.98446 49.97538
0.98471 52.24664
0.98496 54.54602
0.98521 56.86574
0.98546 59.19710
0.98571 61.53055
0.98596 63.85557
0.98622 66.16074
0.98647 68.43371
0.98672 70.66123
0.98697 72.82916
0.98722 74.92252
0.98747 76.92554
0.98772 78.82177
0.98797 80.59413
0.98822 82.22505
0.98847 83.69660
0.98872 84.99067
0.98897 86.08913
0.98922 86.97405
0.98947 87.62793
0.98972 88.03398
0.98997 88.17636
0.99023 88.04053
0.99048 87.61355
0.99073 86.88441
0.99098 85.84440
0.99123 84.48744
0.99148 82.81048
0.99173 80.81379
0.99198 78.50134
0.99223 75.88104
0.99248 72.96508
0.99273 69.77006
0.99298 66.31716
0.99323 62.63218
0.99348 58.74552
0.99373 54.69198
0.99398 50.51052
0.99424 46.24376
0.99449 41.93746
0.99474 37.63971
0.99499 33.40006
0.99524 29.26841
0.99549 25.29379
0.99574 21.52300
0.99599 17.99911
0.99624 14.76002
0.99649 11.83687
0.99674 9.25264
0.99699 7.02092
0.99724 5.14489
0.99749 3.61680
0.99774 2.41788
0.99799 1.51900
0.99825 0.88200
0.99850 0.46195
0.99875 0.21015
0.99900 0.07795
0.99925 0.02094
0.99950 0.00312
0.99975 0.00011
1.00000 0.00000

